Uncertainty Estimation and Calibration with Finite-State Probabilistic RNNs

Uncertainty quantification is crucial for building reliable and trustable machine learning systems. We propose to estimate uncertainty in recurrent neural networks (RNNs) via stochastic discrete state transitions over recurrent timesteps. The uncertainty of the model can be quantified by running a prediction several times, each time sampling from the recurrent state transition distribution, leading to potentially different results if the model is uncertain. Alongside uncertainty quantification, our proposed method offers several advantages in different settings. The proposed method can (1) learn deterministic and probabilistic automata from data, (2) learn well-calibrated models on real-world classification tasks, (3) improve the performance of out-of-distribution detection, and (4) control the exploration-exploitation trade-off in reinforcement learning.

==> author_response.tex <==
Overall:
- Rewrite section 2: clearly separate previous work from ours + recap at the end
- Discuss the two uncertainty types and how our model measures these

AnonReviewer3: nothing additional

AnonReviewer4
- 2.2.: should the dot-product be a matrix-vector product?
- "In (1), t_i does not seem to be defined. Actually, should it not be {t,i}? Additionally, \alpha_i two lines below (2) should be \alpha_{t,i}, presumably.": (Carolin: the time step t is defined. I think {t, i} does make more sense. It also should be \alpha_{t,i}. I modified this in the paper, feel free to undo if you disagree.)

AnonReviewer1:
- "better theoretical justification" on how we capture uncertainty
- How does the uncertanty estimation increase accuracy performance? (Carolin: That makes no sense to me. )
- SOTA methods for each task
- ablation study on their method to figure out what contributes to their method’s improved performance for certain tasks

AnonReviewer2
- use a model that was designed for aleatoric uncertainty
- OOD task: plot of number of states vs. performance
- discuss Hwang et al.

==> sec-background.tex <==
\section{Background and Preliminaries}
\st consists of two building blocks. First, it utilizes state-regularization \citep{WangNiepert:19}, where at each time step a probability distribution over finite set of states is computed. Second, it estimates the probability to transition to each state by learning the temperature of the Gumbel softmax distribution \citep{Gumbel:54,KendallGal:17,JangETAL:17}. This section briefly revisits the two techniques.

\subsection{State-Regularized RNNs}
A Recurrent Neural Network (RNN) computes at each time step $t$ for an input $x_t$ a hidden state $\bfh_t = f\left(\bfh_{t-1},\bfc_{t-1},\bfx_{t}\right)$, where the recurrence is introduced by reusing the hidden state vector $\bfh_{t-1}$ and the cell state $\bfc_{t-1}$ of the previous time step $t-1$.

\srrns~\citep{WangNiepert:19} extend RNNs by dividing the calculation of the hidden state $\bfh_t$ into two components. The first component is the standard recurrent component of a RNN cell
\begin{equation}
\bfu_{t} = f\left(\bfh_{t-1},\bfc_{t-1},\bfx_{t}\right),
\end{equation}
where $\bfu_{t} \in \mathbb{R}^{d}$.
The second component models probabilistic state transitions with $k$ learnable states (or centroids) $\bfs_1$, \dots, $\bfs_k$, which can also be written as a matrix $\mathbf{S} \in \mathbb{R}^{d \times k}$. Based on both components, at each time step, a probability distribution $\bm{\alpha}$ can be defined via a function $g$ (e.g. a softmax transformation),
\begin{equation}\label{eq:alpha2}
\bm{\alpha} = g(\mathbf{S}, \bfu_t).  
\end{equation}

Akin to an attention mechanism \citep{BahdanauETAL:15,VaswaniEATL:17}, individual entries $\alpha_{i}$ of $\bm{\alpha}$ can be understood as the probability that the current vector $\bfu_{t}$ transitions to the corresponding state $\bfs_{i}$.
To arrive at a final hidden state, \citep{WangNiepert:19} compute the probabilistic mixture of the states. However, as this lacks a stochastic component, this cannot directly be used to measure uncertainty. For this, we turn to the Gumbel softmax distribution.


\subsection{The Gumbel-Softmax}
With the Gumbel max trick \citep{Gumbel:54,KendallGal:17,JangETAL:17}, it is possible to draw samples $z$ from a categorical distribution according to a given probability distribution $\pi$, i.e.
\begin{equation}
z= \mbox{\textsc{one\_hot}} \big( \argmax_i [g_i + \log\pi_i] \big), i \in [1\dots k],
\end{equation}
where $k$ is the number of categories and $g_i$ are i.i.d. samples drawn from \textsc{Gumbel}$(0, 1)$, i.e. $g=-\log(-\log(u)), u \sim \textsc{uniform}(0, 1)$. Because the $\argmax$ operator breaks end-to-end differentiability, the categorical distribution $z$ can be approximated using the differentiable softmax function \citep{JangETAL:17,KendallGal:17}. This enables us to draw a $k$-dimensional sample vector $y\in\Delta^{k-1}$ and each instance $y_i$ is assigned a probability, i.e.

\begin{equation}
y_i = \frac{\exp ((\log(\pi_i)+g_i)/\tau)}{\sum_{j=1}^{k} \exp (\log(\pi_j)+g_j)/\tau)}, i \in [1\dots k],
\end{equation}
where $\tau$ is a temperature parameter and $y$ approaches $z$ as $\tau \rightarrow 0$.


